Two-Stage Block Orthogonalization to Improve Performance of $s$-step GMRES

On current computer architectures, GMRES' performance can be limited by its communication cost to generate orthonormal basis vectors of the Krylov subspace. To address this performance bottleneck, its $s$-step variant orthogonalizes a block of $s$ basis vectors at a time, potentially reducing the communication cost by a factor of $s$. Unfortunately, for a large step size $s$, the solver can generate extremely ill-conditioned basis vectors, and to maintain stability in practice, a conservatively small step size is used, which limits the performance of the $s$-step solver. To enhance the performance using a small step size, in this paper, we introduce a two-stage block orthogonalization scheme. Similar to the original scheme, the first stage of the proposed method operates on a block of $s$ basis vectors at a time, but its objective is to maintain the well-conditioning of the generated basis vectors with a lower cost. The orthogonalization of the basis vectors is delayed until the second stage when enough basis vectors are generated to obtain higher performance. Our analysis shows the stability of the proposed two-stage scheme. The performance is improved because while the same amount of computation as the original scheme is required, most of the communication is done at the second stage of the proposed scheme, reducing the overall communication requirements. Our performance results with up to 192 NVIDIA V100 GPUs on the Summit supercomputer demonstrate that when solving a 2D Laplace problem, the two-stage approach can reduce the orthogonalization time and the total time-to-solution by the respective factors of up to $2.6\times$ and $1.6\times$ over the original $s$-step GMRES, which had already obtained the respective speedups of $2.1\times$ and $1.8\times$ over the standard GMRES. Similar speedups were obtained for 3D problems and for matrices from the SuiteSparse Matrix Collection.

==> codes/BCGS2-v3.tex <==
  \begin{algorithmic}[1]
  \Statex \textbf{Input:} $Q_{1:j-1}$
  \Statex \textbf{Output:}  $Q_j$ and $R_{1:j,j}$
     \State {\emph{// Matrix-Powers Kernel}}
     \State $v^{(j)}_1 := q^{(j-1)}_{s+1}$
     \For{$k=1,2,\dots,s$}
        \State $v^{(j)}_{k+1} := A v^{(j)}_{k}$
     \EndFor
       \State {\emph{// First BCGS}}
       \State [$V_{j} $, $T_{1:j-1,j}$] := BCGS($Q_{1:j-1}$, $V_{j}$)
       \State [$V_{j} $, $T_{j,j}$]     := QR($V_{j}$)
       \State {\emph{// Second BCGS}}
       \State [$V_{j} $, $R_{1:j-1,j}$] := BCGS($Q_{1:j-1}$, $V_{j}$)
      \State [$Q_{j},R_{j,j}$] := QR($V_{j}$)
       \State $R_{1:j-1,j} := R_{1:j-1,j} + T_{1:j-1,j}$
       \State $R_{j,j} := R_{j,j} T_{j,j}$
  \end{algorithmic}

==> codes/BCGS2.tex <==
  \begin{algorithmic}[1]
  \Statex \textbf{Input:} $Q_{1:j-1}$ and $V_j$
  \Statex \textbf{Output:}  $Q_j$ and $R_{1:j-1,j}$
        \State {\emph{// BCGS orthogonalization}}
        \State [$V_j$, $R_{1:j-1,j}$] := BCGS($Q_{1:j-1}$, $V_{j}$, $R_{1:j-1,j}$)
        \State {\emph{// BCGS re-orthogonalization}}
        \State [$V_j$, $T_{1:j-1,j}$] := BCGS($Q_{1:j-1}$, $V_{j}$, $R_{1:j-1,j}$)
        \State{\emph{// Update upper-triangular matrix}}
        \State $R_{1:j-1,j} := R_{1:j-1,j} + T_{1:j-1,j}$
  \end{algorithmic}

==> codes/blockQR.tex <==

  \begin{algorithmic}[1]
    \Statex \textbf{Input:} $A$ and $v_0$
    \Statex \textbf{Output:}  $Q$ and $R$
      \For{$j=1,\dots,m/s$}
        \For{$k=1,2,\dots,s$}
           \State $v^{(j)}_{k+1} := A v^{(j)}_{k}$
        \EndFor
        \If {$j > 1$}
          \State {\emph{// BCGS2 orthogonalization}}
          \State [$V_j$, $R_{1:j-1,j}$] := BCGS2($Q_{1:j-1}$, $V_{j}$)
        \EndIf
        \State {\emph{// CholQR2 orthogonalization}}
        \State [$Q_{j}$, $R_{j,j}$] := CholQR2($V_{j}$)
      \EndFor
  \end{algorithmic}

==> codes/cholQR.tex <==
  \begin{algorithmic}[1]
      \Statex \textbf{Input:}  $\widehat{V} \in \mathbb{R}^{n\times s+1}$
      \Statex \textbf{Output:} $Q \in \mathbb{R}^{n\times s+1}$, $R \in \mathbb{R}^{s+1 \times s+1}$
      \State{\emph // Form Gram matrix and compute its Cholesky factorization to gerate $R$}
      \State $G = \widehat{V}^T \widehat{V}$                                         \hspace{5.00cm} (GEMM)
      \State $R = \mbox{chol}(G)$
      \If{Cholesky factorization failed at $k$th step}
        \State{\emph{// Orthogonalize $\widehat{v}_{1:k-1}$ and $\widehat{v}_{k:s+1}$ against $q_{1:k-1}$}}
        \State $q_{1:k-1} := \widehat{v}_{1:k-1}r_{1:k-1,1:k-1}^{-1}$           \hspace{1.85cm} (TRSM)
        \State $\widehat{v}_{k:s+1} := \widehat{v}_{k:s+1} - q_{1:k-1} r_{1:k-1,k:s+1}$   \hspace{0.70cm} (GEMM)
        \State{\emph{// Recursively call CholQR on $v_{k:s+1}$}}
        \State $[q_{k:s+1}, r_{k:s+1,k:s+1}] = \mbox{CholQR}(\widehat{v}_{k:s+1})$
      \Else
        \State{\emph{// Orthogonalize $V$}}
        \State $Q := \widehat{V}R^{-1}$                                         \hspace{4.20cm} (TRSM)
      \EndIf
  \end{algorithmic}

==> letter.tex <==

\onecolumn
\section*{Cover Letter}
Thank you for providing insightful reviews, which were very helpful to improve the quality of our paper.
We have revised the paper to incorporate your comments. We list some of our main changes below, which are also highlighted in blue in the revised paper.

\begin{itemize}
\item We updated our pseudocodes to be more consistent. In particular, we removed MPK from Fig.~\ref{algo:bcgs2} and \ref{algo:bcgs-pip2} such that they now have the same functionality as \textbf{BlkOrtho} in Fig. \ref{algo:sstep}. We decided to keep MPK in Fig.~\ref{algo:2step} since it preprocesses the basis vectors as MPK generates the $s$-step basis vectors.

\item In Section \ref{sec:bcgs2}, we added sentences remarking that the combinations of the inter and intra block-orthogonalization algorithms in Fig.~\ref{algo:bcgs} lead to the orthogonality errors of the computed basis vectors $Q_j$, which can be bounded by $\mathcal{O}(\epsilon)$. In addition, we
formalized a second result, now Theorem IV.2. We believe that this is more clear now
and address the last bullet point of the Committee Comments. 

\item In Section \ref{sec:two-stage}, we extended our discussion (e.g., the third paragraph) to emphasize the impact of the two-stage algorithm on the performance of the block orthogonalization in general setups. We have also added the discussion in the Introduction to clarify these impacts.

\item We have added the second paragraph in Section~\ref{sec:performance} to clarify our choice of the step size $s$ used in our performance studies. We believe that these changes address the second bullet point of the Committee Comments and these changes combined with the above change satisfy the first point.

\item We have added Table~\ref{tab:time-to-sol-shat} to show the performance of the two-stage algorithm
      using different second step sizes $\widehat{s}$. We believe the results further clarify the impacts of the two-stage approach on the solver performance. (This was point 1. of the Committee Comments). Unfortunately, we no longer have access to Summit Supercomputer, where we have conducted our previous performance results. Hence, we have conducted the new performance tests on another testbed (Vortex), which has similar hardware and software specifications. We have observed the solver performance is consistent with our previous results on Summit.
\item We have fixed all the typos that you pointed out. We have also gone through the paper to clarify our discussions and fix additional errors.
\end{itemize}

\bigskip
Thank you again for all of your comments.

\clearpage\newpage
\twocolumn
